A Tale of Two Paradigms: the Mutual Incommensurability of LCDM and MOND

The concordance model of cosmology, LCDM, provides a satisfactory description of the evolution of the universe and the growth of large scale structure. Despite considerable effort, this model does not at present provide a satisfactory description of small scale structure and the dynamics of bound objects like individual galaxies. In contrast, MOND provides a unique and predictively successful description of galaxy dynamics, but is mute on the subject of cosmology. Here I briefly review these contradictory world views, emphasizing the wealth of distinct, interlocking lines of evidence that went into the development of LCDM while highlighting the practical impossibility that it can provide a satisfactory explanation of the observed MOND phenomenology in galaxy dynamics. I also briefly review the baryon budget in groups and clusters of galaxies where neither paradigm provides an entirely satisfactory description of the data. Relatively little effort has been devoted to the formation of structure in MOND; I review some of what has been done. The amplitude ratio of the first to second peak in the CMB power spectrum was correctly predicted a priori, but the third peak is more natural to LCDM. MOND anticipates that structure forms more quickly than in LCDM. This motivated the prediction that reionization would happen earlier in MOND than originally expected in LCDM, as subsequently observed. This also provides a natural explanation for massive, early clusters of galaxies and large, empty voids. However, it is far from obvious that the mass spectrum of galaxy clusters or the power spectrum of galaxies can be explained in MOND, two things that LCDM does well. Critical outstanding issues are the development of an acceptable relativistic parent theory for MOND, and the reality of the non-baryonic dark matter of LCDM. Do suitable dark matter particles exist, or are they a modern aether?

==> abstractforarxiv.tex <==
The concordance model of cosmology, LCDM, provides a satisfactory description of the evolution of the universe and the growth of large scale structure.  Despite considerable effort, this model does not at present provide a satisfactory description of small scale structure and the dynamics of bound objects like individual galaxies.  In contrast, MOND provides a unique and predictively successful description of galaxy dynamics, but is mute on the subject of cosmology.  Here I briefly review these contradictory world views, emphasizing the wealth of distinct, interlocking lines of evidence that went into the development of LCDM while highlighting the practical impossibility that it can provide a satisfactory explanation of the observed MOND phenomenology in galaxy dynamics.  I also briefly review the baryon budget in groups and clusters of galaxies where neither paradigm provides an entirely satisfactory description of the data.  Relatively little effort has been devoted to the formation of structure in MOND; I review some of what has been done.  The amplitude ratio of the first to second peak in the CMB power spectrum was correctly predicted a priori, but the third peak is more natural to LCDM.  MOND anticipates that structure forms more quickly than in LCDM.  This motivated the prediction that reionization would happen earlier in MOND than originally expected in LCDM, as subsequently observed.  This also provides a natural explanation for massive, early clusters of galaxies and large, empty voids.  However, it is far from obvious that the mass spectrum of galaxy clusters or the power spectrum of galaxies can be explained in MOND, two things that LCDM does well.  Critical outstanding issues are the development of an acceptable relativistic parent theory for MOND, and the reality of the non-baryonic dark matter of LCDM.  Do suitable dark matter particles exist, or are they a modern aether?

